Behind the Scenes: An Exploration of Trigger Biases Problem in Few-Shot Event Classification

Few-Shot Event Classification (FSEC) aims at developing a model for event prediction, which can generalize to new event types with a limited number of annotated data. Existing FSEC studies have achieved high accuracy on different benchmarks. However, we find they suffer from trigger biases that signify the statistical homogeneity between some trigger words and target event types, which we summarize as trigger overlapping and trigger separability. The biases can result in context-bypassing problem, i.e., correct classifications can be gained by looking at only the trigger words while ignoring the entire context. Therefore, existing models can be weak in generalizing to unseen data in real scenarios. To further uncover the trigger biases and assess the generalization ability of the models, we propose two new sampling methods, Trigger-Uniform Sampling (TUS) and COnfusion Sampling (COS), for the meta tasks construction during evaluation. Besides, to cope with the context-bypassing problem in FSEC models, we introduce adversarial training and trigger reconstruction techniques. Experiments show these techniques help not only improve the performance, but also enhance the generalization ability of models.

==> alg/alg1.tex <==
\renewcommand{\algorithmicrequire}{ \textbf{Input:}} %Use Input in the format of Algorithm
\renewcommand{\algorithmicensure}{ \textbf{Output:}} %UseOutput in the format of Algorithm

\begin{algorithm}[htb] 
\small
\caption{Confusing Sampling} 
\label{alg:cos}
\begin{algorithmic}[1]
\REQUIRE ~~\\ %算法的输入参数：Input
The number of event in a task, N;\\
The number of instance of each event in a task, K;\\
The number of confusion triggers of an event on anothor event, k; \\
The probability of confusion sampleing, $p_{confusion}$;
\ENSURE ~~\\ %算法的输出：Output
Data of a Task, ${\rm T = \{S, query\}}$;
\STATE {Uniformly sample N events from all events, denoted these events as E}
\STATE ${\rm S} \gets \{\}$
\FOR{all event $e$ $\in$ E}
    \STATE {Cal Alg \ref{alg:cos2} to get confusion and non-confusion trigger set of event $e$}
    \REPEAT
        \STATE $p \gets uniform(0, 1)$
        \IF {$0 \leq p \leq p_{confusion}$}
            \STATE {sample a trigger $t$ from confusion trigger set}
        \ELSE
            \STATE {sample a trigger $t$ from non-confusion trigger set}
        \ENDIF
        \STATE {Sample an instance $i$ of trigger $t$}
        \STATE $S \gets S \cup {i}$
    \UNTIL {K instances belonging to $e$ have been sampled}
\ENDFOR
\STATE {Uniformly sample an event ${\rm e_{query}}$ from E}
\STATE {Sample an instance $i$ of ${\rm e_{query}}$ by step 4 and step 6-12}
\STATE ${\rm{query}} \gets i$
\RETURN {T = \{S, query\}}
\end{algorithmic}
\end{algorithm}



==> alg/alg2.tex <==
\begin{algorithm*}[htb] 
\caption{Pseudocode of triggers partition in a Python-like style} 
\label{alg:Pseuducode} 
\begin{lstlisting}[language=Python]
def partition_triggers(e:str, E:dict, k:int):
"""
Input:
- e: The event that needs to get confusion triggers
- E: all events in the task
- k: the number of confusion triggers of e on each event eo in E-{e}
Return:
- S: non-confusion trigger set
- S_con: confusion trigger set
"""
    # Get all trigger of event e
    T1: dict = allTrigger(e)   
    
    # Calculate the distance triggers of event e
    for t1 in T1: 
        for t2 in T1:
            # d_inner: (T1.size(), T1.size()), Eqn. \ref{con:d_inter}
            d_inner[i][j] = dist(emb(t1), emb(t2)) 
            
    # Get confusion triggers of e on eo
    for eo in E-{e}:
        T2:dict = allTrigger(eo)
      
        # Calculate the distance of triggers between event e and e0
        for t1 in T1:
            for t2 in T2:
                # d_inter: (T1.size(), T2.size()), Eqn. \ref{con:d_inter}
                d_inter[i][j] = dist(emb(t1), emb(t2))
        
        # Calculate mean distance
        for i in range(T1.size()):
            # d_inner: (T1.size())
            d_inner[i] = mean(d_inner[i]) 
            # d_inter: (T1.size())
            d_inter[i] = mean(d_inter[i])  
        
        # Calculate comprehensive distance, Eqn. \ref{con:d_com}
        dist_com = -d_inner + d_inter
      
        # Select k triggers with the smallest comprehensive distance
        indexs = argsort(dist_com)[:k]
      
        # Regard the trigger selected as confusion triggers
        for index in indexs:
            S_con.add(list(T1)[index])
        
    S = T1 - S_con
    return S, S_con
\end{lstlisting}
emb(x): get embedding of token x. \\
dist($\mathbf{v_1}$, $\mathbf{v_2}$): calculate L-2 distance of vector $\mathbf{v_1}$ and $\mathbf{v_2}$. \\
mean($\mathbf{v}$): calculate the average value of  vector $\mathbf{v}$. \\
argsort(L):sort the list L from smallest to largest, and return subscripts instead of values.
\end{algorithm*}


==> alg/alg2c.tex <==
\begin{algorithm*}[htb] 
\caption{Pseudocode of splitting triggers into confusion and non-confusion set in a Python-like style} 
\label{alg:Pseuducode} 
\begin{lstlisting}[language=Python]
def split_triggers(e:str, E:dict, k:int):
"""
Input:
- e: The event that needs to get confusion triggers
- E: all events in the task
- k: the number of confusion triggers of e on each event eo in E-{e}
Return:
- S: non-confusion trigger set
- S_con: confusion trigger set
"""
    # Get all trigger of event e
    T1: dict = allTrigger(e)   
    
    # Calculate the distance triggers of event e
    for t1 in T1: 
        for t2 in T1:
            # d_inner: (T1.size(), T1.size()), Eqn. \ref{con:d_inter}
            d_inner[i][j] = dist(emb(t1), emb(t2)) 
            
    # Get confusion triggers of e on eo
    for eo in E-{e}:
        T2:dict = allTrigger(eo)
      
        # Calculate the distance of triggers between event e and e0
        for t1 in T1:
            for t2 in T2:
                # d_inter: (T1.size(), T2.size()), Eqn. \ref{con:d_inter}
                d_inter[i][j] = dist(emb(t1), emb(t2))
        
        # Calculate mean distance
        for i in range(T1.size()):
            # d_inner: (T1.size())
            d_inner[i] = mean(d_inner[i]) 
            # d_inter: (T1.size())
            d_inter[i] = mean(d_inter[i])  
        
        # Calculate comprehensive distance, Eqn. \ref{con:d_com}
        dist_com = -d_inner + d_inter
      
        # Select k triggers with the smallest comprehensive distance
        indexs = argsort(dist_com)[:k]
      
        # Regard the trigger selected as confusion triggers
        for index in indexs:
            S_con.add(list(T1)[index])
        
    S = T1 - S_con
    return S, S_con
\end{lstlisting}
emb(x): get embedding of token x. \\
dist($\mathbf{v_1}$, $\mathbf{v_2}$): calculate L-2 distance of vector $\mathbf{v_1}$ and $\mathbf{v_2}$. \\
mean($\mathbf{v}$): calculate the average value of  vector $\mathbf{v}$. \\
argsort(L):sort the list L from smallest to largest, and return subscripts instead of values.
\end{algorithm*}


==> table/main_table1.tex <==

\begin{table*}[ht]
\centering
% \small
\caption{Accuracy on MAVEN under different sampling methods for meta tasks construction. We report the average accuracy of $5$ random trials. \textbf{Mean $\Delta$} denotes the mean accuracy difference under TUS/COS in comparison with IUS across $4$ $N$-way-$K$-shot settings. The accuracy of all models dramatically decreases when changing the sampling methods from IUS to TUS/COS.
}
\scalebox{1.0}{
    \begin{tabular}{l|cccccccccccc|cc}
    \toprule
    \multirow{2}{*}{\bf Model} & \multicolumn{3}{c}{\bf 5-way-5-shot} & 
    \multicolumn{3}{c}{\bf 5-way-10-shot} & 
    \multicolumn{3}{c}{\bf 10-way-5-shot} & 
    \multicolumn{3}{c|}{\bf 10-way-10-shot} &
    \multicolumn{2}{c}{\bf Mean \Delta} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
    \cmidrule(lr){14-15}
    ~ & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf TUS & \bf COS   \\
    \midrule
    String Match  &  61.06 & 19.82 & 19.59 & 71.85 & 19.65 & 19.19 & 55.36 & 9.82 & 9.69 & 67.19 & 9.63 & 9.39 & -49.14 & -49.40 \\
    GloVe Match &  84.96 & 59.71 & 45.70 & 88.62 & 66.65 & 52.44 & 78.22 & 45.8 & 35.03 & 82.67 & 52.68 & 42.35 & -27.41 & -39.74 \\
    \midrule
    % MN  &  00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00  & -00.00 & -00.00\\
    Proto-CNN  &  82.44 & 57.15 & 46.19 & 86.49 & 62.60 & 53.21 & 74.92 & 42.73 & 34.67 & 78.87 & 48.21 & 41.53 & -28.01 & -36.78 \\
    Proto-BiLSTM  & 85.61 & 60.95 & 49.04 & 88.65 & 67.43 & 56.54 & 78.95 & 46.43 & 37.09 & 82.80 & 53.72 & 44.62 & -26.87 & -37.18 \\
    HATT & 84.08 & 57.60 & 45.90 & 87.77 & 63.32 & 52.23 & 76.41 & 42.98 & 34.31 & 81.33 & 49.59 & 41.17 & -29.02 & -39.00 \\
    HATT+LoLoss  & 84.98 & 57.65 & 46.51 & 88.82 & 64.49 & 54.13 & 77.72 & 44.02 & 35.00 & 82.62 & 50.71 & 41.33 & -29.32 & -39.29 \\
    HATT+Loss$_{\mathrm{int}}$  & 83.75 & 57.02 & 46.47 & 87.93 & 64.06 & 52.40 & 76.10 & 42.58 & 34.23 & 81.55 & 49.00 & 40.81 & -29.17 & -38.86 \\
    \midrule
    Proto-BERT  & 90.48 & 69.31 & 60.46 & 92.37 & 75.30 & 68.06 & 84.89 & 55.91 & 47.81 & 87.95 & 62.65 & 56.38 & -23.13 & -30.75 \\
    HATT-BERT  &  90.07 & 65.01 & 55.56 & 92.94 & 71.73 & 61.38 & 85.17 & 51.94 & 43.14 & 88.09 & 58.95 & 49.15 & -27.16 & -36.76 \\
    \bottomrule
    \end{tabular}
}
\label{table:maven-main}
\end{table*}


==> table/main_table2.tex <==
\begin{table*}[htbp]
\centering
% \small
\caption{Accuracy on FewEvent under different sampling methods for meta tasks construction. We report the average accuracy of $5$ random trials. \textbf{Mean $\Delta$} denotes the mean accuracy difference under TUS/COS in comparison with IUS across $4$ $N$-way-$K$-shot settings. The accuracy of all models dramatically decreases when changing the sampling methods from IUS to TUS/COS.
}
\scalebox{1.0}{
    \begin{tabular}{l|cccccccccccc|cc}
    \toprule
    \multirow{2}{*}{\bf Model} & \multicolumn{3}{c}{\bf 5-way-5-shot} & 
    \multicolumn{3}{c}{\bf 5-way-10-shot} & 
    \multicolumn{3}{c}{\bf 10-way-5-shot} & 
    \multicolumn{3}{c|}{\bf 10-way-10-shot} &
    \multicolumn{2}{c}{\bf Mean \Delta} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
    \cmidrule(lr){14-15}
    ~ & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf TUS & \bf COS   \\
    \midrule
    String Match  & 68.51 & 19.51 & 19.36 & 77.29 & 19.13 & 18.97 & 64.47 & 9.46 & 9.38 & 74.37 & 9.12 & 8.97 & -56.86 & -56.99 \\
    GloVe Match &   84.90 & 57.88 & 54.54 & 87.57 & 61.81 & 60.70 & 79.10 & 46.15 & 43.27 & 83.02 & 50.26 & 48.21 & -29.62 & -31.97 \\
    \midrule
    % MN  &  00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00  & -00.00 & -00.00\\
    Proto-CNN  & 81.09 & 61.84 & 60.50 & 84.21 & 63.60 & 63.58 & 71.95 & 48.75 & 48.15 & 77.80 & 51.54 & 50.12 & -22.33 & -23.18 \\
    Proto-BiLSTM  &  86.86 & 63.43 & 59.70 & 89.06 & 66.70 & 65.55 & 80.06 & 50.12 & 46.49 & 84.09 & 54.11 & 51.67 & -26.43 & -29.17 \\
    HATT  &  82.95 & 64.30 & 59.76 & 85.24 & 66.33 & 64.75 & 75.24 & 51.94 & 47.35 & 79.47 & 55.09 & 52.75 & -21.31 & -24.57 \\
    HATT+LoLoss  &  83.40 & 64.50 & 62.54 & 87.35 & 67.04 & 66.82 & 76.88 & 51.33 & 49.80 & 80.47 & 55.17 & 54.89 & -22.52 & -23.51 \\
    HATT+Loss_{\mathrm{int}}  & 82.69 & 64.60 & 62.36 & 86.15 & 65.84 & 65.17 & 74.85 & 51.09 & 48.48 & 79.84 & 54.95 & 52.47 & -21.76 & -23.76 \\
    \midrule
    Proto-BERT  &  94.01 & 78.89 & 78.22 & 95.24 & 80.61 & 81.75 & 90.83 & 69.85 & 69.94 & 93.03 & 72.58 & 74.83 & -17.80 & -17.09 \\
    HATT-BERT  &  94.96 & 80.01 & 77.75 & 95.44 & 79.16 & 79.77 & 90.86 & 70.84 & 68.05 & 92.72 & 68.73 & 68.92 & -18.81 & -19.87 \\
    \bottomrule
    \end{tabular}
}
\label{table:fewevent-main}
\end{table*}


==> table/table34.tex <==

\begin{table*}
\caption{Accuracy under $4$ different $N$-way-$K$-shot settings. We report the average accuracy of $5$ random trials. Using adversarial training (+adv) and trigger reconstruction (+rec) leads to improvements under different sampling methods for evaluation.}
\centering
 
\subtable[\textbf{Results on FewEvent Dataset.}]{
\scalebox{1.0}{
    \begin{tabular}{l|cccccccccccc}
    \toprule
    \multirow{2}{*}{\bf Model} & \multicolumn{3}{c}{\bf 5-way-5-shot} & 
    \multicolumn{3}{c}{\bf 5-way-10-shot} & 
    \multicolumn{3}{c}{\bf 10-way-5-shot} & 
    \multicolumn{3}{c}{\bf 10-way-10-shot} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
    ~ & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS   \\
    \midrule
    Proto-CNN  & 81.09 & 61.84 & 60.5 & 84.21 & 63.6 & 63.58 & 71.95 & 48.75 & 48.15 & 77.8 & 51.54 & 50.12 \\
    +adv  & 81.30 & 65.49 & 63.42 & \bf 85.92 & 66.95 & 66.04 & 73.19 & 51.77 & 51.45 & 78.72 & 54.55 & \bf 54.59 \\
    +rec  & \bf 83.12 & 64.78 & 63.57 & 85.31 & 65.61 & 64.04 & 72.71 & 51.41 & 50.39 & 79.07 & 53.89 & 52.70 \\
    +adv+rec  & 82.49 & \bf 65.83 & \bf 65.09 & 85.83 & \bf 68.35 & \bf 67.40 & \bf 73.53 & \bf 52.84 & \bf 52.27 & \bf 79.66 & \bf 55.28 & 53.68 \\
    \midrule
    Proto-BERT   & 94.01 & 78.89 & 78.22 & 95.24 & 80.61 & 81.75 & 90.83 & 69.85 & 69.94 & 93.03 & 72.58 & 74.83 \\
    +adv  & 94.31 & 79.81 & 79.28 & 95.64 & 82.07 & 82.81 & 91.22 & \bf 71.91 & 70.86 & \bf 93.52 & 74.44 & 76.01 \\
    +rec  & 94.17 & 79.14 & 78.63 & 95.61 & 81.26 & 82.80 & 91.18 & 71.26 & 70.87 & 93.24 & 73.07 & 75.45 \\
    +adv+rec  & \bf 94.45 & \bf 79.87 & \bf 79.62 & \bf 95.75 & \bf 82.80 & \bf 83.18 & \bf 91.57 & 71.73 & \bf 72.30 & 93.25 & \bf 75.03 & \bf 76.35  \\
    \bottomrule
    \end{tabular}
}

\label{table:fewevent-adv-rec}
}
 
\subtable[\textbf{Results on MAVEN Dataset.}]{        
\scalebox{1.0}{
    \begin{tabular}{l|cccccccccccc}
    \toprule
    \multirow{2}{*}{\bf Model} & \multicolumn{3}{c}{\bf 5-way-5-shot} & 
    \multicolumn{3}{c}{\bf 5-way-10-shot} & 
    \multicolumn{3}{c}{\bf 10-way-5-shot} & 
    \multicolumn{3}{c}{\bf 10-way-10-shot} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
    ~ & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS & \bf IUS & \bf TUS & \bf COS   \\
    \midrule
     Proto-CNN  &   82.44 & 57.15 & 46.19 & 86.49 & 62.60 & 53.21 & 74.92 & 42.73 & 34.67 & 78.87 & 48.21 & 41.53 \\
    +adv & 83.39 & 58.54 & 48.05 & \bf 87.63 & 64.44 & \bf 55.44 & 76.22 & 44.09 & 35.55 & \bf 80.58 & 50.86 & 42.83 \\
    +rec  & 83.35 & 56.94 & 47.19 & 87.03 & 63.37 & 53.63 & 75.36 & 43.41 & 35.23 & 79.90 & 49.04 & 42.07 \\
    +adv+rec  & \bf 83.90 & \bf 58.93 & \bf 48.26 & 87.58 & \bf 64.96 & 55.21 & \bf 76.27 & \bf 44.34 & \bf 36.12 & 80.30 & \bf 51.06 & \bf 43.06 \\
    \midrule
    Proto-BERT & 90.48 & 69.31 & 60.46 & 92.37 & 75.30 & 68.06 & 84.89 & 55.91 & 47.81 & 87.95 & 62.65 & 56.38 \\
    +adv  & 90.67 & 69.89 & 60.68 & 92.74 & 75.43 & 69.71 & 85.93 & 56.89 & 49.07 & 88.11 & \bf 64.12 & 57.70 \\
    +rec  & 90.59 & 69.70 & 60.51 & 92.24 & 75.43 & 68.59 & 85.32 & 56.84 & 48.71 & 88.01 & 63.90 & 57.48 \\
    +adv+rec  & \bf 90.80 & \bf 70.70 & \bf 61.30 & \bf 92.82 & \bf 76.03 & \bf 70.06 & \bf 86.00 & \bf 57.18 & \bf 49.44 & \bf 88.34 & 64.11 & \bf 57.72 \\
    \bottomrule
    \end{tabular}
}
\label{table:maven-adv-rec}
}
 
\end{table*}
